High-Fidelity Qutrit Entangling Gates for Superconducting Circuits

Ternary quantum information processing in superconducting devices poses a promising alternative to its more popular binary counterpart through larger, more connected computational spaces and proposed advantages in quantum simulation and error correction. Although generally operated as qubits, transmons have readily addressable higher levels, making them natural candidates for operation as quantum three-level systems (qutrits). Recent works in transmon devices have realized high fidelity single qutrit operation. Nonetheless, effectively engineering a high-fidelity two-qutrit entanglement remains a central challenge for realizing qutrit processing in a transmon device. In this work, we apply the differential AC Stark shift to implement a flexible, microwave-activated, and dynamic cross-Kerr entanglement between two fixed-frequency transmon qutrits, expanding on work performed for the $ZZ$ interaction with transmon qubits. We then use this interaction to engineer efficient, high-fidelity qutrit CZ$^\dag$ and CZ gates, with estimated process fidelities of 97.3(1)% and 95.2(3)% respectively, a significant step forward for operating qutrits on a multi-transmon device.

==> supp_preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
\usepackage{xcolor}


% \usepackage[pdftex, pdftitle={Article}, pdfauthor={Author}]{hyperref} % 

% \hypersetup{
%     colorlinks=true,
%     linkcolor=red,
%     filecolor=magenta,      
%     urlcolor=cyan,
% }
\usepackage{xcolor}
\usepackage{cleveref} % smart reference
\newcommand{\alexis}[1]{{\textsf{{\color{red}{Alexis' comment:}   #1 }}}}

% Tikz
\usepackage{tikz}

\renewcommand{\a}{{\alpha}}



\usepackage[normalem]{ulem} % For \sout

% Joel's macros
\newcommand{\mc}{\mathcal}
\newcommand{\bb}{\mathbb}
\newcommand{\cn}{{\textcolor{blue}{[citation needed]}}}

\newcommand{\dbra}[1]{\ensuremath{\langle\!\langle #1|}}
\newcommand{\dket}[1]{\ensuremath{|#1\rangle\!\rangle}}

%from https://stackoverflow.com/a/1812477/3183467
\makeatletter
\def\dketbra#1{\def\tempa{#1}\futurelet\next\dketbra@i}% Save first argument
\def\dketbra@i{\ifx\next\bgroup\expandafter\dketbra@ii\else\expandafter\dketbra@end\fi}%Check brace
\def\dketbra@ii#1{| \tempa \rangle\!\rangle\!\langle\!\langle #1 |}%Two args
\def\dketbra@end{| \tempa \rangle\!\rangle\!\langle\!\langle \tempa |}%Single args
\makeatother

\makeatletter
\def\dbraket#1{\def\tempa{#1}\futurelet\next\dbraket@i}% Save first argument
\def\dbraket@i{\ifx\next\bgroup\expandafter\dbraket@ii\else\expandafter\dbraket@end\fi}%Check brace
\def\dbraket@ii#1{\langle\!\langle \tempa | #1 \rangle\!\rangle}%Two args
\def\dbraket@end{\langle\!\langle \tempa | \tempa \rangle\!\rangle}%Single args
\makeatother

